Zero-shot Generative Large Language Models for Systematic Review Screening Automation

Systematic reviews are crucial for evidence-based medicine as they comprehensively analyse published research findings on specific questions. Conducting such reviews is often resource- and time-intensive, especially in the screening phase, where abstracts of publications are assessed for inclusion in a review. This study investigates the effectiveness of using zero-shot large language models~(LLMs) for automatic screening. We evaluate the effectiveness of eight different LLMs and investigate a calibration technique that uses a predefined recall threshold to determine whether a publication should be included in a systematic review. Our comprehensive evaluation using five standard test collections shows that instruction fine-tuning plays an important role in screening, that calibration renders LLMs practical for achieving a targeted recall, and that combining both with an ensemble of zero-shot models saves significant screening time compared to state-of-the-art approaches.

==> results-table-fusion.tex <==
\begin{tabular}{ll|llllllll}
	\toprule
	Dataset  & Model &Precision& Recall &B-AC&F0.5& F1& F3 &P(R90)&WSS\\
	\hline \addlinespace[2pt]
CLEF-2017 & fused & 0.077 & 0.920 & 0.726 & 0.093 & 0.134 & 0.353 & 0.055 & 0.516 \\
\midrule
CLEF-2018 & fused & 0.089 & 0.937 & 0.739 & 0.106 & 0.149 & 0.369 & 0.063 & 0.520 \\
\midrule
CLEF-2019-dta & fused & 0.104 & 0.881 & 0.727 & 0.118 & 0.153 & 0.329 & 0.027 & 0.552 \\
\midrule
CLEF-2019-intervention & fused & 0.082 & 0.918 & 0.699 & 0.097 & 0.137 & 0.344 & 0.049 & 0.463 \\
\midrule
Seed Collection & fused & 0.059 & 0.896 & 0.662 & 0.071 & 0.102 & 0.281 & 0.036 & 0.417 \\
\midrule
\end{tabular}


==> results-table-in-ex.tex <==
\begin{tabular}{ll|llllllll}
	\toprule
	
	Dataset& Model &Precision& Recall &B-AC&F0.5& F1& F3 &P(R90)& WSS \\
	\hline \addlinespace[2pt]
	clef-tar-CLEF-2017& llama-2-chat & 0.074 & 0.860 & 0.726 & 0.089 & 0.128 & 0.333 & 0.050 & 0.577 \\
	clef-tar-CLEF-2017& llama-2-chat & 0.061 & 0.910 & 0.666 & 0.074 & 0.108 & 0.306 & 0.042 & 0.411 \\\midrule
	clef-tar-CLEF-2017& llama-2-13b-chat & 0.185 & 0.397 & 0.660 & 0.184 & 0.201 & 0.292 & 0.005 & 0.912 \\
	clef-tar-CLEF-2017& llama-2-13b-chat & 0.241 & 0.338 & 0.647 & 0.224 & 0.225 & 0.284 & 0.000 & 0.944 \\\midrule
	
	clef-tar-CLEF-2018& llama-2-chat & 0.094 & 0.882 & 0.748 & 0.111 & 0.154 & 0.368 & 0.033 & 0.594 \\
	clef-tar-CLEF-2018& llama-2-chat & 0.102 & 0.880 & 0.711 & 0.118 & 0.158 & 0.356 & 0.052 & 0.521 \\\midrule
	clef-tar-CLEF-2018& llama-2-13b-chat & 0.257 & 0.364 & 0.659 & 0.245 & 0.249 & 0.303 & 0.000 & 0.940 \\
	clef-tar-CLEF-2018& llama-2-13b-chat & 0.333 & 0.362 & 0.666 & 0.285 & 0.273 & 0.321 & 0.019 & 0.958 \\\midrule
	
	clef-tar-CLEF-2019-dta& llama-2-chat & 0.092 & 0.922 & 0.714 & 0.109 & 0.149 & 0.346 & 0.072 & 0.492 \\
	clef-tar-CLEF-2019-dta& llama-2-chat & 0.088 & 0.924 & 0.676 & 0.103 & 0.142 & 0.340 & 0.073 & 0.416 \\\midrule
	clef-tar-CLEF-2019-dta& llama-2-13b-chat & 0.192 & 0.490 & 0.688 & 0.199 & 0.220 & 0.318 & 0.000 & 0.870 \\
	clef-tar-CLEF-2019-dta& llama-2-13b-chat & 0.226 & 0.427 & 0.661 & 0.224 & 0.233 & 0.301 & 0.000 & 0.880 \\\midrule
	
	clef-tar-CLEF-2019-intervention& llama-2-chat & 0.081 & 0.903 & 0.704 & 0.097 & 0.138 & 0.351 & 0.051 & 0.490 \\
	clef-tar-CLEF-2019-intervention& llama-2-chat & 0.087 & 0.875 & 0.692 & 0.103 & 0.145 & 0.358 & 0.031 & 0.493 \\\midrule
	clef-tar-CLEF-2019-intervention& llama-2-13b-chat & 0.181 & 0.476 & 0.682 & 0.186 & 0.213 & 0.343 & 0.005 & 0.873 \\
	clef-tar-CLEF-2019-intervention& llama-2-13b-chat & 0.263 & 0.524 & 0.716 & 0.256 & 0.281 & 0.397 & 0.019 & 0.888 \\\midrule
\end{tabular}


==> results-table-seed.tex <==
\begin{tabular}{ll|lllllll}
	\toprule
	
	Dataset& Model &Precision& Recall &B-AC&F0.5& F1& F3 &P(R90) \\
	\hline \addlinespace[2pt]
	%below for zero-shot
sysrev-seed-collection& llama & 0.036 & 0.871 & 0.467 & 0.044 & 0.066 & 0.209 & 0.029 \\
sysrev-seed-collection& llama-2 & 0.042 & 0.278 & 0.530 & 0.049 & 0.066 & 0.143 & 0.000 \\
sysrev-seed-collection& llama-2-13b & 0.037 & \textbf{0.975} & 0.489 & 0.045 & 0.068 & 0.222 & 0.037 \\
sysrev-seed-collection& falcon & 0.037 & 0.905 & 0.487 & 0.045 & 0.067 & 0.216 & 0.031 \\
sysrev-seed-collection& alpaca & 0.037 & 0.875 & 0.485 & 0.045 & 0.067 & 0.212 & 0.029 \\
sysrev-seed-collection& llama-2-chat & 0.052 & 0.881 & 0.646 & 0.063 & 0.092 & 0.268 & 0.036 \\
sysrev-seed-collection& llama-2-13b-chat & \textbf{0.124} & 0.467 & \textbf{0.666} & \textbf{0.128} & \textbf{0.150} & \textbf{0.272} & 0.002 \\
	\midrule
	%below for  average seed
sysrev-seed-collection& llama-seed & 0.035 & 0.868 & 0.467 & 0.043 & 0.065 & 0.207 & 0.027 \\
sysrev-seed-collection& llama-2-seed & 0.038 & 0.648 & 0.501 & 0.046 & 0.068 & 0.195 & 0.016 \\
sysrev-seed-collection& llama-2-13b-seed & 0.039 & 0.891 & 0.516 & 0.048 & 0.071 & 0.224 & 0.031 \\
sysrev-seed-collection& falcon-seed & 0.037 & 0.816 & 0.479 & 0.044 & 0.065 & 0.191 & 0.017 \\
sysrev-seed-collection& alpaca-seed & 0.021 & 0.316 & 0.269 & 0.026 & 0.036 & 0.096 & 0.007 \\
sysrev-seed-collection& llama-2-chat-seed & 0.039 & \textbf{0.893} & 0.514 & 0.048 & 0.072 & 0.226 & \textbf{0.031} \\
sysrev-seed-collection& llama-2-13b-chat-seed & \textbf{0.109} & 0.433 & \textbf{0.639} & \textbf{0.109} & \textbf{0.127} & \textbf{0.231} & 0.009 \\
	
	
	\midrule
	
%below for optimal seed for optimising B-AC
sysrev-seed-collection& llama-seed & 0.038 & 0.908 & 0.516 & 0.047 & 0.070 & 0.222 & 0.031 \\
sysrev-seed-collection& llama-2-seed & 0.047 & 0.744 & 0.589 & 0.057 & 0.083 & 0.231 & 0.026 \\
sysrev-seed-collection& llama-2-13b-seed & 0.044 & \textbf{0.914} & 0.577 & 0.054 & 0.079 & 0.243 & 0.030 \\
sysrev-seed-collection& falcon-seed & 0.040 & 0.854 & 0.512 & 0.048 & 0.069 & 0.201 & 0.020 \\
sysrev-seed-collection& alpaca-seed & 0.045 & 0.615 & 0.554 & 0.054 & 0.077 & 0.209 & 0.011 \\
sysrev-seed-collection& llama-2-chat-seed & 0.047 & 0.898 & 0.609 & 0.058 & 0.086 & 0.261 & \textbf{0.035} \\
sysrev-seed-collection& llama-2-13b-chat-seed & \textbf{0.145} & 0.651 & \textbf{0.748} & \textbf{0.156} & \textbf{0.194} & \textbf{0.374} & 0.014 \\
	
	\bottomrule
\end{tabular}
